A universal black-box optimization method with almost dimension-free convergence rate guarantees

Universal methods for optimization are designed to achieve theoretically optimal convergence rates without any prior knowledge of the problem's regularity parameters or the accurarcy of the gradient oracle employed by the optimizer. In this regard, existing state-of-the-art algorithms achieve an $\mathcal{O}(1/T^2)$ value convergence rate in Lipschitz smooth problems with a perfect gradient oracle, and an $\mathcal{O}(1/\sqrt{T})$ convergence rate when the underlying problem is non-smooth and/or the gradient oracle is stochastic. On the downside, these methods do not take into account the problem's dimensionality, and this can have a catastrophic impact on the achieved convergence rate, in both theory and practice. Our paper aims to bridge this gap by providing a scalable universal gradient method - dubbed UnderGrad - whose oracle complexity is almost dimension-free in problems with a favorable geometry (like the simplex, linearly constrained semidefinite programs and combinatorial bandits), while retaining the order-optimal dependence on $T$ described above. These "best-of-both-worlds" results are achieved via a primal-dual update scheme inspired by the dual exploration method for variational inequalities.

==> App-Examples.tex <==
%----------------------------------------------------------------------
%%% APP: BREGMAN
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


In this appendix, we provide some details for the calculations concerning the examples presented in \cref{sec:base}.


%----------------------------------------------------------------------
%%% Simplex
%----------------------------------------------------------------------
\subsection*{\cref{ex:simplex}: Simplex setup}

The regularizer of choice in \cref{ex:simplex} is the negative entropy $\hreg(\load) = \sum_{\resource} \load_{\resource} \log\load_{\resource}$ which has $\range = \log\vdim$.
By the definition of the problem, if $\cost_{\resource}(\load_{\resource}) \leq \boundcoord_{0}$ and $\cost_{\resource}'(\load_{\resource}) \leq \boundcoord_{1}$ for all $\load_{\resource} \in [0,1]$, $\resource = 1,\dotsc,\nResources$, it follows that the problem's objective satisfies \eqref{eq:BG} relative to the $L^{\infty}$ norm on $\R^{\vdim}$ with $\gbound_{\infty} = \boundcoord_{0} + \boundcoord_{1}$.
Since $\hreg$ is $1$-strongly convex relative to the $L^{1}$ norm (see e.g., Example 2.5. of \cite{SS11}),
\PM{What's the best reference for this?}\DQV{Is Shalev-Schwartz'11 
OK?}
the convergence rate \eqref{eq:MP-BG} of \eqref{eq:MP} only carries an $\bigof*{\sqrt{\log\vdim}}$ dependence on the problem's dimension (and likewise if each $\cost_{\resource}$ is twice differentiable). 

By contrast, if we were to use the Euclidean regularizer $\hreg(\load) = \sum_{\resource} \load_{\resource}^{2}/2$, we would have $\range \leq 2$.
However, since $\onenorm{\cdot} \leq \sqrt{\vdim} \twonorm{\cdot}$ with equality achieved at the barycenter of the simplex, the corresponding strong convexity constant for $\hreg$ would be $\hstr = 1/\vdim$.
As a result, the convergence rate \eqref{eq:MP-BG} for the Euclidean version of \eqref{eq:MP} \textendash\ that is, the \acl{EG} algorithm \textendash\ would scale as $\bigoh(\sqrt{\vdim})$ in terms of the problem's dimensionality.


%----------------------------------------------------------------------
%%% Spectrahedron
%----------------------------------------------------------------------
\subsection*{\cref{ex:spectron}: Spectrahedron setup}

A tailor-made regularizer for the spectrahedron is the von Neumann entropy
\begin{equation}
\hreg(\covmat)
	= \tr\bracks{\covmat \log\covmat}
	+ (1 - \tr\covmat) \log(1-\tr\covmat).
\end{equation}
As we discuss in the appendix, $\hreg$ is $1$-strongly convex relative to the nuclear norm $\onenorm{\covmat} = \tr\sqrt{\covmat\covmat^{\dag}}$ on $\points$;
moreover, the Shannon\textendash Telatar capacity \eqref{eq:capa} satisfies \eqref{eq:BG} with $\gbound = \max\eig(\chanmat^{\dag}\chanmat)$ relative to the spectral norm $\norm{\cdot}_{\infty}$ on the space of Hermitian matrices.
Since $\range = \log\nInput = (1/2)\log\vdim$, the dependence of the convergence rate of \eqref{eq:MP} on $\vdim$ is again $\bigof*{\sqrt{\log\vdim}}$.


%----------------------------------------------------------------------
%%% Combinatorial
%----------------------------------------------------------------------
\subsection*{\cref{ex:comband}: Combinatorial setup}

Following \cite{LS20}, consider the unnormalized entropic regularizer $\hreg(\point) = \sum_{\coord=1}^{\vdim} \parens{\point_{\coord} \log\point_{\coord} - \point_{\coord}}$ restricted to $\points = \conv(\pures)$.


==> App-Sequences.tex <==
%----------------------------------------------------------------------
%%% APP: SEQUENCES
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


In this appendix, we provide some necessary inequalities on numerical sequences that we require for the convergence rate analysis of the previous sections.
Most of the lemmas presented below already exist in the literature, and go as far back as \citet{ACBG02} and \citet{MS10};
when appropriate, we note next to each lemma the references with the statement closest to the precise version we are using in our analysis.
These lemmas can also be proved by the general methodology outlined in \citet[Lem.~14]{GSE14}, so we only provide a proof for two ancillary results that would otherwise require some more menial bookkeeping.

\smallskip

%This first lemma that we present is due to \cite{MS10} and \cite{LYC18}.

\begin{lemma}[\citealp{MS10}, \citealp{LYC18}]
\label{lem:sqrt}
For all non-negative numbers $\alpha_{1},\dotsc \alpha_{\run}$, the following inequality holds:
\begin{equation}
\sqrt{\sum_{\run=1}^{\nRuns}\alpha_{\run}}\leq \sum_{\run=1}^{\nRuns}\dfrac{\alpha_{\run}}{\sqrt{\sum_{i=1}^{\run}\alpha_{i}}}\leq 2\sqrt{\sum_{\run=1}^{\nRuns}\alpha_{\run}}
\end{equation}
\end{lemma}

%\begin{proof}
%We begin, by introducing some necessary notation and set $S=\sum_{\run=1}^{\nRuns}\alpha_{\run}$ and $\point=\alpha_{\nRuns}$.
%
%The first part is proved by induction. The induction base case $\nRuns=1$ straightforwardly holds. Now for the induction step, assume that the lemma holds for $\nRuns-1$ and we will show that it holds for $\nRuns$ as well.
%In particular, we have:
%\begin{align}
%\sum_{\run=1}^{\nRuns}\dfrac{\alpha_{\run}}{\sqrt{\sum_{i=1}^{\run}\alpha_{i}}}
%	&= \sum_{\run=1}^{\nRuns-1}\dfrac{\alpha_{\run}}{\sqrt{\sum_{i=1}^{\run}\alpha_{i}}}
%		+\dfrac{\alpha_{\nRuns}}{\sqrt{\sum_{\run=1}^{\nRuns}\alpha_{\run}}}
%	\notag\\
%	&\geq \sqrt{\sum_{\run=1}^{\nRuns-1}\alpha_{\run}}
%		+ \dfrac{\alpha_{\nRuns}}{\sqrt{\sum_{\run=1}^{\nRuns}\alpha_{\run}}}
%	%\notag\\
%	=\sqrt{S-\point}+\frac{x}{\sqrt{S}}
%\end{align}
%where the first inequality is obtained due to the induction hypothesis. Hence, in order to prove the lemma
%it is sufficient to show that:
%\begin{equation}
%\sqrt{S-\point}+\frac{x}{\sqrt{S}}\geq \sqrt{S}
%\end{equation}
%By multiplying both sides by $\sqrt{S}$, we get the following equivalent expression:
%\begin{equation}
%\sqrt{S^{2}-\point S}\geq S-\point
%\end{equation}
%whereas after rearranging we obtain the equivalent inequality:
%\begin{equation}
%\point\leq S
%\end{equation}
%which holds, since $\point=\alpha_{\nRuns}\leq \sum_{\run=1}^{\nRuns}\alpha_{\run}=S$ and hence the \acs{LHS}
%inequality is obtained.
%\\
%Now, the proof of the \acs{RHS} inequality:
%\begin{equation}
%\sum_{\run=1}^{\nRuns}\dfrac{\alpha_{\run}}{\sqrt{\sum_{i=1}^{\run}\alpha_{i}}}\leq 2\sqrt{\sum_{\run=1}^{\nRuns}\alpha_{\run}}
%\end{equation}
%will again be done again via induction. The induction base $\nRuns=1$ holds immediately.
%Assume that the lemma holds for $\nRuns-1$. We will show that it also holds for $\nRuns$. By the induction hypothesis, we get:
%\begin{equation}
%\sum_{\run=1}^{\nRuns}\dfrac{\alpha_{\run}}{\sqrt{\sum_{i=1}^{\run}\alpha_{i}}}\leq 2\sqrt{\sum_{\run=1}^{\nRuns-1}\alpha_{\run}}+ \dfrac{\alpha_{\nRuns}}{\sqrt{\sum_{\run=1}^{\nRuns}\alpha_{\run}}}
%=2\sqrt{S-\point}+\frac{\point}{\sqrt{S}}
%\end{equation}
%where $\point=\alpha_{\nRuns}$ and $S=\sum_{\run=1}^{\nRuns}\alpha_{\run}$ (we highlight once more that $\point\leq S$). Taking the derivative of the function $H(x)=2\sqrt{S-\point}+\frac{\point}{\sqrt{S}}$ (with respect to $\point$), we get that:
%\begin{equation}
%H'(\point)= \frac{1}{\sqrt{S}}-\frac{1}{\sqrt{S-\point}}
%\end{equation}
%becomes negative for all $\point \geq 0$. Thus, $H(x)\leq H(0)=2\sqrt{S}$ and therefore the result follows.
%\end{proof}

\begin{lemma}[\citealp{LYC18}]
\label{lem:logarithmic-1}
For all non-negative numbers $\alpha_{1},\dotsc \alpha_{\run}$, the following inequality holds:
\begin{equation}
\sum_{\run=1}^{\nRuns}\dfrac{\alpha_{\run}}{1+\sum_{i=1}^{\run}\alpha_{i}}\leq 1+\log(1+\sum_{\run=1}^{\nRuns}\alpha_{\run})
\end{equation}
\end{lemma}

%\begin{proof}
%The lemma will proved by induction. The induction base $\nRuns=1$ holds, since:
%\begin{equation}
%\frac{\alpha_{1}}{1+\alpha_{1}}\leq 1\leq 1+\log(1+\alpha_{1})
%\end{equation}
%Assume now that the lemma holds for $\nRuns-1$. Then, we are left to show that it also holds for $\nRuns$.
%Indeed, by the induction hypothesis, we get:
%\begin{equation}
%\sum_{\run=1}^{\nRuns}\dfrac{\alpha_{\run}}{1+\sum_{i=1}^{\run}\alpha_{i}}\leq 1+\log(1+\sum_{\run=1}^{\nRuns-1}\alpha_{\run})+\frac{\alpha_{\nRuns}}{1+\sum_{\run=1}^{\nRuns}\alpha_{\run}}
%\end{equation}
%Thus, in order to complete the induction it suffices to show that:
%\begin{equation}
%1+\log(1+\sum_{\run=1}^{\nRuns-1}\alpha_{\run})+\frac{\alpha_{\nRuns}}{1+\sum_{\run=1}^{\nRuns}\alpha_{\run}}\leq 1+\log(1+\sum_{\run=1}^{\nRuns}\alpha_{\run})
%\end{equation}
%By denoting $\point=\alpha_{\nRuns}/(1+\sum_{\run=1}^{\nRuns-1}\alpha_{\run})$, the above equation is equivalent:
%\begin{equation}
%\log(\point+1)-\frac{\point}{1+\point}\geq 0
%\end{equation}
%which can be straighforwardly checked since $H(\point)=\log(\point+1)-\frac{\point}{1+\point}\leq 0$ for all $\point \geq 0$. Therefore, the result follows.
%\end{proof}

\begin{lemma}
\label{lem:logarithmic-2}
Let $b_{1},\dotsc, b_{\run}$ a sequence of non-negative numbers with $b_{1}>0$. Then, the following inequality holds:
\begin{equation}
\sum_{\run=1}^{\nRuns}
	\dfrac{b_{\run}}{\sum_{i=1}^{\run}b_{i}}
	\leq 2+\log\parens*{\dfrac{\sum_{\run=1}^{\nRuns}b_{\run}}{b_{1}}}
\end{equation}
\end{lemma}
\begin{proof}
It is directly obtained by applying \cref{lem:logarithmic-1} for the sequence $\alpha_{\run}=b_{\run}/b_{1}$.
\end{proof}

The following set of inequalities are due to \cite{BL19}. For completeness, we provide a sketch of their proof.

\begin{lemma}[\citealp{BL19}]
\label{lem:ineq}
For all non-negative numbers: $\alpha_{1},\dotsc \alpha_{\run}\in [0,\alpha]$, $\alpha_{0}\geq 0$, the following inequality holds:
\begin{equation}
\sqrt{\alpha_{0}+\sum_{\run=1}^{\nRuns-1}\alpha_{i}}-\sqrt{\alpha_{0}}\leq \sum_{\run=1}^{\nRuns}\frac{\alpha_{\run}}{\sqrt{\alpha_{0}+\sum_{i=1}^{\run-1}\alpha_{j}}}\leq \frac{2\alpha}{\sqrt{\alpha_{0}}}+3\sqrt{\alpha}+3\sqrt{\alpha_{0}+\sum_{\run=1}^{\nRuns-1}\alpha_{\run}}
\end{equation}
\end{lemma}

%\begin{proof}
%We will show the first part of the inequality:
%\begin{equation}
%\sqrt{\alpha_{0}+\sum_{\run=1}^{\nRuns-1}\alpha_{i}}-\sqrt{\alpha_{0}}\leq \sum_{\run=1}^{\nRuns}\frac{\alpha_{\run}}{\sqrt{\alpha_{0}+\sum_{i=1}^{\run-1}\alpha_{j}}}
%\end{equation}
%by induction. The induction base $\nRuns=1$ is true since in this case we get:
%\begin{equation}
%\sum_{\run=1}^{1}\frac{\alpha_{\run}}{\sqrt{\alpha_{0}+\sum_{i=1}^{\run-1}\alpha_{j}}}= \frac{\alpha_{1}}{\sqrt{\alpha_{0}}}\geq \sqrt{\alpha_{0}+\alpha_{1}}-\sqrt{\alpha_{0}}
%\end{equation}
%which becomes equivalent with the formulation
%\begin{equation}
%(\alpha_{0}+\alpha_{1})^{2}\geq \alpha_{0}(\alpha_{0}+\alpha_{1})
%\end{equation}
%which holds since $\alpha_{0},\alpha_{1}\geq 0$.
%\\
%For the induction step assume that it holds for $\nRuns-1$ and we will show that it holds also for $\nRuns$.
%In particular, by the induction hypothesis we have:
%\begin{equation}
%\sum_{\run=1}^{\nRuns}\frac{\alpha_{\run}}{\sqrt{\alpha_{0}+\sum_{j=1}^{\run-1}}}\geq \sqrt{\alpha_{0}+\sum_{\run=1}^{\nRuns-1}\alpha_{\run}}-\sqrt{\alpha_{0}}+\frac{\alpha_{\nRuns}}{\alpha_{0}+\sum_{\run=1}^{\nRuns-1}\alpha_{\run}}
%\end{equation}
%Now, by denoting $\point=\alpha_{\nRuns}$ and $Z=\alpha_{0}+\sum_{\run=1}^{\nRuns}\alpha_{\run}$ we get the equivalent expression:
%\begin{equation}
%\sum_{\run=1}^{\nRuns}\frac{\alpha_{\run}}{\sqrt{\alpha_{0}+\sum_{j=1}^{\run-1}}}\geq \sqrt{Z-\point}+\frac{\point}{\sqrt{Z-\point}}-\sqrt{\alpha_{0}}
%\end{equation}
%Hence, in order to complete the proof it is sufficient to show that:
%\begin{equation}
%\sqrt{Z-\point}+\frac{\point}{\sqrt{Z-\point}}\geq \sqrt{Z}
%\end{equation}
%Indeed, if we consider the function $H(\point)=\sqrt{Z-\point}+\frac{\point}{\sqrt{Z-\point}}$ we can directly derive that it is monotonically increasing on $[0,Z]$ (note that $\point \leq Z$).
%So, we have:
%\begin{equation}
%\sqrt{Z-\point}+\frac{\point}{\sqrt{Z-\point}}=H(\point)\geq H(0)=\sqrt{Z}
%\end{equation}
%For the second part of the inequality:
%\begin{equation}
% \sum_{\run=1}^{\nRuns}\frac{\alpha_{\run}}{\sqrt{\alpha_{0}+\sum_{i=1}^{\run-1}\alpha_{j}}}\leq \frac{2\alpha}{\sqrt{\alpha_{0}}}+3\sqrt{\alpha}+3\sqrt{\alpha_{0}+\sum_{\run=1}^{\nRuns-1}\alpha_{\run}}
%\end{equation}
%We distiguish two cases: If $\alpha \leq \alpha_{0}$ then it is clear.
%For the other case, where $\alpha_{0}\leq \alpha$, we denote:
%\begin{equation}
%\nRuns_{0}=\min\{\run \in [\nRuns]: \sum_{j=1}^{\run-1}\alpha_{j}\geq \alpha\}
%\end{equation}
%We divide the sum according to $\nRuns_{0}$:
%\begin{align}
%\sum_{\run=1}^{\nRuns}\frac{\alpha_{\run}}{\sqrt{\alpha_{0}+\sum_{j=1}^{\run-1}\alpha_{j}}}&=
%\sum_{\run=1}^{\nRuns_{0}-1}\frac{\alpha_{\run}}{\sqrt{\alpha_{0}+\sum_{j=1}^{\run-1}\alpha_{j}}}
%+ \sum_{\run=\nRuns_{0}}^{\nRuns}\frac{\alpha_{\run}}{\sqrt{\alpha_{0}+\sum_{j=1}^{\run-1}\alpha_{j}}}
%\notag\\
%&\leq \frac{2\alpha}{\sqrt{\alpha_{0}}}+\sqrt{2}\sum_{\run=\nRuns_{0}}^{\nRuns}\frac{\alpha_{\run}}{\sqrt{\alpha +\sum_{j=\nRuns_{0}}^{\run-1}\alpha_{j}}}
%\notag\\
%&\leq \frac{2\alpha}{\sqrt{\alpha_{0}}}+3\sqrt{\alpha}+3\sqrt{\alpha_{0}+\sum_{\run=1}^{\nRuns-1}\alpha_{\run}}
%	\end{align}
%	where we used $\sum_{j=1}^{\nRuns_{0}-2}\alpha_{j}\leq \alpha$, as well as well as for all $\run \geq \nRuns_{0}, \sum_{j=1}^{\run-1}\alpha_{j}\geq \alpha$ (both follow from the definition of $\nRuns_{0}$)
%\end{proof}

\begin{lemma}
\label{lem:logarithmic-3}
For all non-negative numbers: $\alpha_{1},\dotsc \alpha_{\run}\in [0,\alpha]$, $\alpha_{0}\geq 0$, we have:
\begin{equation}
\sum_{\run=1}^{\nRuns}\frac{\alpha_{\run}}{\alpha_{0}+\sum_{i=1}^{\run-1}\alpha_{i}}
	\leq 2
		+ \frac{4\alpha}{\alpha_{0}}
		+ 2\log\parens*{1+\sum_{\run=1}^{\nRuns-1}\frac{\alpha_{\run}}{\alpha_{0}}}
\end{equation}
\end{lemma}

\begin{proof}
Let us denote
\begin{equation}
\txs
\nRuns_{0}
	= \min \setdef[\big]{\run \in [\nRuns]}{\sum_{j=1}^{\run-1}\alpha_{j}\geq \alpha}
\end{equation}
Then, dividing the sum by $\nRuns_{0}$, we get:
\begin{align}
\sum_{\run=1}^{\nRuns}\frac{\alpha_{\run}}{\alpha_{0}+\sum_{i=1}^{\run-1}\alpha_{i}}&
	\leq \sum_{\run=1}^{\nRuns_{0}-1}\frac{\alpha_{\run}}{\alpha_{0}+\sum_{i=1}^{\run-1}\alpha_{i}}  
	+\sum_{\run=\nRuns_{0}}^{\nRuns}\frac{\alpha_{\run}}{\alpha_{0}+\sum_{i=1}^{\run-1}\alpha_{i}}
	\notag\\
	&\leq \frac{1}{\alpha_{0}}\sum_{\run=1}^{\nRuns_{0}-1}\alpha_{\run}+\sum_{\run=\nRuns_{0}}^{\nRuns}
	\dfrac{\alpha_{\run}}{1/2\alpha_{0}+1/2\alpha+1/2\sum_{j=1}^{\run-1}\alpha_{j}}
	\notag\\
	&\leq \frac{\alpha}{\alpha_{0}}+2\sum_{\run=\nRuns_{0}}^{\nRuns}\dfrac{\alpha_{i}/\alpha_{0}}{1+\sum_{j=\nRuns_{0}}^{\run}\alpha_{j}/\alpha_{0}}
	\notag\\
	&\leq \frac{2\alpha}{\alpha_{0}}
		+ 2
		+ 2\log\parens*{1+\sum_{\run=\nRuns_{0}}^{\nRuns}\alpha_{i}/\alpha_{0}}
	\notag\\
	&\leq \frac{2\alpha}{\alpha_{0}}
		+ 2
		+ 2\log\parens*{1 + \sum_{\run=1}^{\nRuns}\alpha_{i}/\alpha_{0}}
\end{align}
where we used the fact that $\sum_{j=1}^{\nRuns_{0}-2}\alpha_{j}\leq \alpha$ as well as for all $\run \geq \nRuns_{0}, \sum_{j=1}^{\run-1}\alpha_{j}\geq \alpha$ (both follow from the definition of $\nRuns_{0}$) and \cref{lem:logarithmic-1}.
\end{proof}

==> Proof.tex <==
%----------------------------------------------------------------------
%%% PROOF
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


Let \mbox{$	\reg_{\nRuns} \defeq \sum_{\run=1}^{\nRuns}{\curr[\step]}\inner{\nabla \obj \parens*{\half{\state}{\run}}}{\half{\state}{\run}-\sol}$}, the starting point of our proof is the following result: %
\begin{equation}
	\ex \bracks*{\gap \parens{{\nRuns}}} \leq {2 \ex \bracks*{\reg_{\nRuns} }} \big/ {\nRuns^{2}} \textrm{ for any } \nRuns. \label{eq:lem:proof_adaEW}
\end{equation}
%
\eqref{eq:lem:proof_adaEW} is a standard result in working with the $\curr[\step]$-weighted averaging technique that also appears in several previous works \citep{cutkosky2019anytime,KLBC19}. 

Note that in \eqref{eq:opt}, under the first-order oracle, $\nabla \obj \parens*{\half{\state}{\run}}$ is \emph{not} observed (instead, only $\half{\signal}{\nRuns}$ is observable). Therefore, instead of working with $\reg_{\nRuns}$, we focus on the term $\regstoch_{\nRuns} \defeq  \sum_{\run=1}^{\nRuns} {\curr[\step]}\inner*{ \half{\signal}{\nRuns} }{\half{\state}{\run}-\sol}$.


\begin{proposition}\label{prop:energy_inequ}
\DQV{@Kim, please change when you have the precise proof.}	Run \method, for any $\point \in \points$, we have:
	\begin{align}
		\regstoch_{\nRuns} %
		\le & \hreg(\sol) -  \min \hreg +   \const \sum \nolimits_{\run=1}^{\nRuns}  (\curr[\step])^2 \learn^{\run+1} \dnorm{\curr[\signal]-\curr[\testsignal]}^{2} \nonumber \\
		%
		& \vspace{+2cm} - \sum \nolimits_{\run=1}^{\nRuns}  \norm{\curr[\precom]-\curr[\ptest]}^{2} \big/ \parens*{2\strong \next[\learn] } , \label{eq:Propo_energy_inequ}
	\end{align}
where $\const \defeq {\hreg(\sol) -  \min \hreg +\frac{\strong^2 + 2\diam^2}{2\strong} }$.
\end{proposition} 


\paragraph{Novelty of \cref{prop:energy_inequ}.} \cref{prop:energy_inequ} is a key element leading to desired results in \cref{thm:stoch}. This is due to the following reasons:


\begin{proof}[Proof of \cref{prop:energy_inequ}]
@Kim
\end{proof}






Let us define the noises of the observed feedback at each time epoch:
 \begin{equation*}
 	\curr[\noise] \defeq \curr[\signal] - \nabla \obj \parens*{\curr[\avg{\state}]} \textrm{ and } \half{\noise}{\run} \defeq \half{\signal}{\run} - \nabla \obj \parens*{ \avghalf{\state}{\run} }. 
 \end{equation*} 
%
%  From these definitions, we also deduce that $\ex \bracks*{\noisetest^{\run} \middle| \prev[\mathcal{H}] }  = \ex \bracks*{\noise^{\run} \middle|\prev[\mathcal{H}]} = \zer$ where $\prev[\mathcal{H}] = \braces*{ \state^{\run-1}, \test^{\run-1}, \sample^{\run-1}, \ldots, \state^{\start},\test^{\start}, \sample^{\start} } $ is the filtration up to time epoch $\run-1$. 
 %
% \cref{eq:Propo_energy_inequ} involves the difference of the actual gradients of the BMW potential $\nabla \obj( \curr[\state])-\nabla \obj(\avg{\state})$ and the difference of costs at $\state$ and $\test$, \ie $\obs^{\run}-\obsave^{\run}$ (in the static case, these differences are equal).
We also define the following terms:
% in order to analyze the gap between these differences:
\begin{align*}
	 & \curr[\mindiff]=\min\braces*{\dnorm{ \nabla \obj(\avghalf{\state}{\run}) -  \nabla \obj(\curr[\avg{\state}]) }^{2},\dnorm{\half{\signal}{\run}  - \curr[\signal]  }^{2}}, \\
	 %
	 & \curr[\diff]=\bracks*{\half{\signal}{\run}  - \curr[\signal] } - \bracks*{ \nabla \obj(\avghalf{\state}{\run}) -  \nabla \obj(\curr[\avg{\state}]) }.
\end{align*}












%
%
%%%%%%%%%%
From \cref{prop:energy_inequ}, under different settings (smooth/ non-smooth), we can derive various results stated in the following proposition:
%
\begin{proposition}\label{prop:diff}
%
Let $\conststoch \defeq \hreg(\sol) -  \min \hreg +\frac{\strong^2 + 3\diam^2}{2\strong}$. Under the \LSmCon Condition, we~have:
\begin{align}
	\regstoch_{\nRuns} \le & \hreg(\sol) -  \min\hreg +  \conststoch 2\sqrt{2} \parens*{\sum_{\run=1}^{\nRuns}(\curr[\step])^{2} \dnorm{\curr[\diff]}^{2}}^{1/2} \nonumber \\
	%
	    & \hspace{1cm} + 32 \smooth \conststoch^{3/2} \sqrt{2 \strong}. \label{eq:diff_LSm}
\end{align}

Under the \BdCon Condition, we~have:
\begin{align}
	\regstoch_{\nRuns} \le & \ldots \label{eq:diff_Bd}
\end{align}
\end{proposition}

The proof of \cref{prop:diff} is based on the fact that the second and the third term in \eqref{eq:Propo_energy_inequ} are actually summable. Moreover, by our \emph{special choice of adaptive sequence of learning rate} $\curr[\learn]$, the sum of these terms is of order $\bigoh(1)$ since only a constant number of components in this summation are positive.
Due to the space constraints, we relegate the proof of \cref{prop:diff} to Appendix~\ref{app:proofs}.


Finally, note that $\ex \bracks*{  \dnorm{\curr[\diff]}^{2}} \le    2\ex \bracks*{  \dnorm{ \noise^{\run}  }^{2}} +  2\ex \bracks*{  \dnorm{  \noiseave^{\run}   }^{2}} \le  4 \sdev^2$ ( by the definition of $\sdev$, $\sup \braces*{\exof*{\dnorm{\half{\noise}{\run}}}, \exof*{\dnorm{\curr[\noise]}} } \le \sdev$), we derive \eqref{eq:Stoch_Smooth} by taking expectation of the two sides of \eqref{eq:diff_LSm} and derive \eqref{eq:Stoch_Bd} by taking taking expectation of the two sides of \eqref{eq:diff_Bd}.
